A Systematic Study on Weak Galerkin Finite Element Method for Second Order Parabolic Problems

A systematic numerical study on weak Galerkin (WG) finite element method for second order linear parabolic problems is presented by allowing polynomial approximations with various degrees for each local element. Convergence of both semidiscrete and fully discrete WG solutions are established in $L^{\infty}(L^2)$ and $L^{\infty}(H^1)$ norms for a general WG element $({\cal P}_{k}(K),\;{\cal P}_{j}(\partial K),\;\big[{\cal P}_{l}(K)\big]^2)$, where $k\ge 1$, $j\ge 0$ and $l\ge 0$ are arbitrary integers. The fully discrete space-time discretization is based on a first order in time Euler scheme. Our results are intended to extend the numerical analysis of WG methods for elliptic problems [J. Sci. Comput., 74 (2018), 1369-1396] to parabolic problems. Numerical experiments are reported to justify the robustness, reliability and accuracy of the WG finite element method.

==> WG_Para_Sys_Ref_MMM.tex <==
@article{dehghan2006computational,
	title={A computational study of the one-dimensional parabolic equation subject to nonclassical boundary specifications},
	author={Dehghan, Mehdi},
	journal={Numerical Methods for Partial Differential Equations},
	volume={22},
	number={1},
	pages={220--257},
	year={2006},
	publisher={Wiley Online Library}
}




@article{dehghan2007one,
	title={The one-dimensional heat equation subject to a boundary integral specification},
	author={Dehghan, Mehdi},
	journal={Chaos, Solitons \& Fractals},
	volume={32},
	number={2},
	pages={661--675},
	year={2007},
	publisher={Elsevier}
}



@article{abbaszadeh2020meshless,
	title={Meshless local numerical procedure based on interpolating moving least squares approximation and exponential time differencing fourth-order Runge--Kutta (ETDRK4) for solving stochastic parabolic interface problems},
	author={Abbaszadeh, Mostafa and Dehghan, Mehdi},
	journal={Engineering with Computers},
	pages={1--21},
	year={2020},
	publisher={Springer}
}


@article{dehghan2006numerical,
	title={Numerical solution of two-dimensional parabolic equation subject to nonstandard boundary specifications using the pseudospectral Legendre method},
	author={Dehghan, Mehdi and Shamsi, M},
	journal={Numerical Methods for Partial Differential Equations},
	volume={22},
	number={6},
	pages={1255--1266},
	year={2006},
	publisher={Wiley Online Library}
}


@article{dehghan2005efficient,
	title={Efficient techniques for the second-order parabolic equation subject to nonlocal specifications},
	author={Dehghan, Mehdi},
	journal={Applied Numerical Mathematics},
	volume={52},
	number={1},
	pages={39--62},
	year={2005},
	publisher={Elsevier}
}

@article{dehghan2002new,
	title={A new ADI technique for two-dimensional parabolic equation with an integral condition},
	author={Dehghan, M},
	journal={Computers \& Mathematics with Applications},
	volume={43},
	number={12},
	pages={1477--1488},
	year={2002},
	publisher={Elsevier}
}


@incollection{raviart1977mixed,
  title={A mixed finite element method for 2-nd order elliptic problems},
  author={Raviart, Pierre-Arnaud and Thomas, Jean-Marie},
  booktitle={Mathematical aspects of finite element methods},
  pages={292--315},
  year={1977},
  publisher={Springer}
}
@book{brenner2007mathematical,
  title={The mathematical theory of finite element methods},
  author={Brenner, Susanne and Scott, Ridgway},
  volume={15},
  year={2007},
  publisher={Springer Science \& Business Media}
}

@article{mu2020pressure,
  title={Pressure Robust Weak Galerkin Finite Element Methods for Stokes Problems},
  author={Mu, Lin},
  journal={SIAM Journal on Scientific Computing},
  volume={42},
  number={3},
  pages={B608--B629},
  year={2020},
  publisher={SIAM}
}

@article{mu2020uniformly,
  title={A Uniformly Robust H (DIV) Weak Galerkin Finite Element Methods for Brinkman Problems},
  author={Mu, Lin},
  journal={SIAM Journal on Numerical Analysis},
  volume={58},
  number={3},
  pages={1422--1439},
  year={2020},
  publisher={SIAM}
}

@article{liu2020penalty,
  title={Penalty-Free Any-Order Weak Galerkin FEMs for Elliptic Problems on Quadrilateral Meshes},
  author={Liu, Jiangguo and Tavener, Simon and Wang, Zhuoran},
  journal={Journal of Scientific Computing},
  volume={83},
  pages={47},
  year={2020},
  publisher={Springer}
}

@article{brezzi1985two,
  title={Two families of mixed finite elements for second order elliptic problems},
  author={Brezzi, Franco and Douglas, Jim and Marini, L Donatella},
  journal={Numerische Mathematik},
  volume={47},
  number={2},
  pages={217--235},
  year={1985},
  publisher={Springer}
}

@book{thomee1990finite,
  title={Galerkin finite element methods for parabolic problems},
  author={Thom{\'e}e, Vidar},
  volume={1054},
  year={1984},
  publisher={Springer}
}

@article{wang2013weak,
	title={A weak \mbox{Galerkin} finite element method for second-order elliptic problems},
	author={Wang, Junping and Ye, Xiu},
	journal={Journal of Computational and Applied Mathematics},
	volume={241},
	pages={103--115},
	year={2013},
	publisher={Elsevier}
}

@article{wang2014weak,
	title={A weak \mbox{Galerkin} mixed finite element method for second order elliptic problems},
	author={Wang, Junping and Ye, Xiu},
	journal={Mathematics of Computation},
	volume={83},
	number={289},
	pages={2101--2126},
	year={2014}
}

@article{wang2018systematic,
	title={A systematic study on weak \mbox{Galerkin} finite element methods for second order elliptic problems},
	author={Wang, Junping and Wang, Ruishu and Zhai, Qilong and Zhang, Ran},
	journal={Journal of Scientific Computing},
	volume={74},
	number={3},
	pages={1369--1396},
	year={2018},
	publisher={Springer}
}

@article{li2018interior,
	title={Interior energy error estimates for the weak \mbox{Galerkin} finite element method},
	author={Li, Hengguang and Mu, Lin and Ye, Xiu},
	journal={Numerische Mathematik},
	volume={139},
	number={2},
	pages={447--478},
	year={2018},
	publisher={Springer}
}


@article{wang2018primal,
	title={A primal-dual weak \mbox{Galerkin} finite element method for second order elliptic equations in non-divergence form},
	author={Wang, Chunmei and Wang, Junping},
	journal={Mathematics of Computation},
	volume={87},
	number={310},
	pages={515--545},
	year={2018}
}

@article{mu2017least,
	title={A Least-Squares-Based Weak \mbox{Galerkin} Finite Element Method for Second Order Elliptic Equations},
	author={Mu, Lin and Wang, Junping and Ye, Xiu},
	journal={SIAM Journal on Scientific Computing},
	volume={39},
	number={4},
	pages={A1531--A1557},
	year={2017},
	publisher={SIAM}
}

@article{lin2018weak,
	title={A Weak \mbox{Galerkin} Finite Element Method for Singularly Perturbed Convection-Diffusion--Reaction Problems},
	author={Lin, Runchang and Ye, Xiu and Zhang, Shangyou and Zhu, Peng},
	journal={SIAM Journal on Numerical Analysis},
	volume={56},
	number={3},
	pages={1482--1497},
	year={2018},
	publisher={SIAM}
}

@article{liu2018lowest,
	title={Lowest-order weak \mbox{Galerkin} finite element method for Darcy flow on convex polygonal meshes},
	author={Liu, Jiangguo and Tavener, Simon and Wang, Zhuoran},
	journal={SIAM Journal on Scientific Computing},
	volume={40},
	number={5},
	pages={B1229--B1252},
	year={2018},
	publisher={SIAM}
}

@article{xie2019error,
	title={Error analysis of weak \mbox{Galerkin} finite element methods for time-dependent convection--diffusion equations},
	author={Xie, Shenglan and Zhu, Peng and Wang, Xiaoshen},
	journal={Applied Numerical Mathematics},
	volume={137},
	pages={19--33},
	year={2019},
	publisher={Elsevier}
}

@article{zhang2016weak,
	title={Weak \mbox{Galerkin} finite element method for second order parabolic equations},
	author={Zhang, Hongqin and Zou, Yongkui and Xu, Yingxiang and Zhai, Qilong and Yue, Hua},
	journal={Int. J. Numer. Anal. Model},
	volume={13},
	number={4},
	pages={525--544},
	year={2016}
}

@article{li2013weak,
	title={Weak \mbox{Galerkin} finite element methods for parabolic equations},
	author={Li, Qiaoluan H and Wang, Junping},
	journal={Numerical Methods for Partial Differential Equations},
	volume={29},
	number={6},
	pages={2004--2024},
	year={2013},
	publisher={Wiley Online Library}
}

@article{zhou2019weak,
	title={Weak \mbox{Galerkin} finite element method with second-order accuracy in time for parabolic problems},
	author={Zhou, Shiping and Gao, Fuzheng and Li, Benxing and Sun, Zhengjia},
	journal={Applied Mathematics Letters},
	volume={90},
	pages={118--123},
	year={2019},
	publisher={Elsevier}
}

@article{wang2016discretization,
	title={Discretization of div--curl systems by weak \mbox{Galerkin} finite element methods on polyhedral partitions},
	author={Wang, Chunmei and Wang, Junping},
	journal={Journal of Scientific Computing},
	volume={68},
	number={3},
	pages={1144--1171},
	year={2016},
	publisher={Springer}
}

@article{wang2016weak,
	title={A weak \mbox{Galerkin} finite element method for the Stokes equations},
	author={Wang, Junping and Ye, Xiu},
	journal={Advances in Computational Mathematics},
	volume={42},
	number={1},
	pages={155--174},
	year={2016},
	publisher={Springer}
}

@article{zhang2019globally,
	title={A globally divergence-free weak \mbox{Galerkin} method for Brinkman equations},
	author={Zhang, Li and Feng, Minfu and Zhang, Jian},
	journal={Applied Numerical Mathematics},
	volume={137},
	pages={213--229},
	year={2019},
	publisher={Elsevier}
}


@article{mu2015weak,
	title={A weak \mbox{Galerkin} finite element method for the Maxwell equations},
	author={Mu, Lin and Wang, Junping and Ye, Xiu and Zhang, Shangyou},
	journal={Journal of Scientific Computing},
	volume={65},
	number={1},
	pages={363--386},
	year={2015},
	publisher={Springer}
}

@article{shields2017weak,
	title={Weak \mbox{Galerkin} methods for time-dependent Maxwell's equations},
	author={Shields, Sidney and Li, Jichun and Machorro, Eric A},
	journal={Computers \& Mathematics with Applications},
	volume={74},
	number={9},
	pages={2106--2124},
	year={2017},
	publisher={Elsevier}
}

@article{liu2016weak,
	title={A weak \mbox{Galerkin} finite element method for the Oseen equations},
	author={Liu, Xin and Li, Jian and Chen, Zhangxin},
	journal={Advances in Computational Mathematics},
	volume={42},
	number={6},
	pages={1473--1490},
	year={2016},
	publisher={Springer}
}

@article{mu2018weak,
	title={A Weak \mbox{Galerkin} Method for the Reissner--Mindlin Plate in Primary Form},
	author={Mu, Lin and Wang, Junping and Ye, Xiu},
	journal={Journal of Scientific Computing},
	volume={75},
	number={2},
	pages={782--802},
	year={2018},
	publisher={Springer}
}


@article{deka2019weak,
  title={Weak \mbox{Galerkin} Finite Element Methods for Parabolic Interface Problems with Nonhomogeneous Jump Conditions},
  author={Deka, Bhupen and Roy, Papri},
  journal={Numerical Functional Analysis and Optimization},
  volume={40},
  number={3},
  pages={259--279},
  year={2019},
  publisher={Taylor \& Francis}
}

@article{song2018relaxed,
	title={A relaxed weak \mbox{Galerkin} method for elliptic interface problems with low regularity},
	author={Song, Lunji and Zhao, Shan and Liu, Kaifang},
	journal={Applied Numerical Mathematics},
	volume={128},
	pages={65--80},
	year={2018},
	publisher={Elsevier}
}

@article{mu2016new,
	title={A new weak \mbox{Galerkin} finite element method for elliptic interface problems},
	author={Mu, Lin and Wang, Junping and Ye, Xiu and Zhao, Shan},
	journal={Journal of Computational Physics},
	volume={325},
	pages={157--173},
	year={2016},
	publisher={Elsevier}
}

@book{ciarlet2002finite,
  title={The finite element method for elliptic problems},
  author={Ciarlet, Philippe G},
  volume={40},
  year={2002},
  publisher={Siam}
}

@article{vacca2015virtual,
  title={Virtual element methods for parabolic problems on polygonal meshes},
  author={Vacca, Giuseppe and Beir{\~a}o da Veiga, Lourenco},
  journal={Numerical Methods for Partial Differential Equations},
  volume={31},
  number={6},
  pages={2110--2134},
  year={2015},
  publisher={Wiley Online Library}
}

@article{da2014virtual,
  title={A virtual element method with arbitrary regularity},
  author={da Veiga, Lourenco Beir{\~a}o and Manzini, Gianmarco},
  journal={IMA Journal of Numerical Analysis},
  volume={34},
  number={2},
  pages={759--781},
  year={2014},
  publisher={Oxford university press}
}

@article{beirao2013basic,
  title={Basic principles of virtual element methods},
  author={Beir{\~a}o da Veiga, L and Brezzi, Franco and Cangiani, Andrea and Manzini, Gianmarco and Marini, L Donatella and Russo, Alessandro},
  journal={Mathematical Models and Methods in Applied Sciences},
  volume={23},
  number={01},
  pages={199--214},
  year={2013},
  publisher={World Scientific}
}

@article{cangiani2014hp,
  title={hp-version discontinuous \mbox{Galerkin} methods on polygonal and polyhedral meshes},
  author={Cangiani, Andrea and Georgoulis, Emmanuil H and Houston, Paul},
  journal={Mathematical Models and Methods in Applied Sciences},
  volume={24},
  number={10},
  pages={2009--2041},
  year={2014},
  publisher={World Scientific}
}

@article{cangiani2017hp,
  title={hp-version space-time discontinuous Galerkin methods for parabolic problems on prismatic meshes},
  author={Cangiani, Andrea and Dong, Zhaonan and Georgoulis, Emmanuil H},
  journal={SIAM Journal on Scientific Computing},
  volume={39},
  number={4},
  pages={A1251--A1279},
  year={2017},
  publisher={SIAM}
}

@article{cockburn2009unified,
  title={Unified hybridization of discontinuous Galerkin, mixed, and continuous Galerkin methods for second order elliptic problems},
  author={Cockburn, Bernardo and Gopalakrishnan, Jayadeep and Lazarov, Raytcho},
  journal={SIAM Journal on Numerical Analysis},
  volume={47},
  number={2},
  pages={1319--1365},
  year={2009},
  publisher={SIAM}
}
@article{wang2019basics,
  title={The basics of weak Galerkin finite element methods},
  author={Wang, Junping and Ye, Xiu},
  journal={arXiv preprint arXiv:1901.10035},
  year={2019}
}

@article{cockburn2018weak,
  title={The Weak Galerkin methods are rewritings of the Hybridizable Discontinuous Galerkin methods},
  author={Cockburn, Bernardo},
  journal={arXiv preprint arXiv:1812.08146},
  year={2018}
}

@article{cockburn2016bridging,
  title={Bridging the hybrid high-order and hybridizable discontinuous Galerkin methods},
  author={Cockburn, Bernardo and Di Pietro, Daniele A and Ern, Alexandre},
  journal={ESAIM: Mathematical Modelling and Numerical Analysis},
  volume={50},
  number={3},
  pages={635--650},
  year={2016},
  publisher={EDP Sciences}
}

@article{arnold2002unified,
  title={Unified analysis of discontinuous Galerkin methods for elliptic problems},
  author={Arnold, Douglas N and Brezzi, Franco and Cockburn, Bernardo and Marini, L Donatella},
  journal={SIAM journal on numerical analysis},
  volume={39},
  number={5},
  pages={1749--1779},
  year={2002},
  publisher={SIAM}
}

@article{doi:10.1137/S0036142900377991,
	author = {Chrysafinos, K. and Hou, L. S.},
	title = {Error Estimates for Semidiscrete Finite Element Approximations of Linear and Semilinear Parabolic Equations Under Minimal Regularity Assumptions},
	journal = {SIAM Journal on Numerical Analysis},
	volume = {40},
	number = {1},
	pages = {282-306},
	year = {2002},
	doi = {10.1137/S0036142900377991},
	
}

@book{ra,
  title={Sobolev Spaces, sec. ed},
  author={Adams, RA and Fournier, JJF},
  year={2003},
  publisher={Academic Press, Amsterdam}
}

@book{necas1996weak,
  title={Weak and measure-valued solutions to evolutionary PDEs},
   author={M\'{e}lek, J and Ne\v{c}as, J  and Rokyta, M and R{u}\v{z}i\v{c}ka, M},
  volume={13},
  year={1996},
  publisher={Chapman \& Hall, London, UK}
}

@Article{IJNAM-12-31,
	author = {Lin Mu and Junping Wang & Xiu Ye},
	title = {Weak \mbox{Galerkin} Finite Element Methods on Polytopal Meshes},
	journal = {International Journal of Numerical Analysis and Modeling},
	year = {2015},
	volume = {12},
	number = {1},
	pages = {31--53},
	issn = {2617-8710},
	doi = {https://doi.org/}
}

@article{dai,
  title={A mathematical model for skin burn injury induced by radiation heating},
  author={Dai, Weizhong and Wang, Haojie and Jordan, Pedro M and Mickens, Ronald E and Bejan, Adrian},
  journal={International Journal of Heat and Mass Transfer},
  volume={51},
  number={23-24},
  pages={5497--5510},
  year={2008},
  publisher={Elsevier}
}

@article{pen,
title={Analysis of tissue and arterial temperature in the resting human forearm},
author={Pennes, H. H.},
journal={J. Appl. Physiol.},
volume={1},
number={2},
pages={93--122},
year={1948},
publisher={APS}
}

@article{chen1998finite,
  title={Finite element methods and their convergence for elliptic and parabolic interface problems},
  author={Chen, Zhiming and Zou, Jun},
  journal={Numerische Mathematik},
  volume={79},
  number={2},
  pages={175--202},
  year={1998},
  publisher={Springer}
}

